Mis\`ere Games and Mis\`ere Quotients

These lecture notes are based on a short course on mis\`ere quotients offered at the Weizmann Institute of Science in Rehovot, Israel, in November 2006. They include an introduction to impartial games, starting from the beginning; the basic mis\`ere quotient construction; a proof of the Guy--Smith--Plambeck Periodicity Theorem; and statements of some recent results and open problems in the subject.

==> macros.tex <==
\makeatletter

\newcommand{\present}[4][c]{
  \parbox[#1]{#2}{\raggedright $\<#3~|~\misere@buildpresent#4,@\>$}
}

\newcommand{\hangingpresent}[4][c]{
  \begin{array}[#1]{@{}c@{~}c@{~}p{#2}@{}}
  \<#3 & | & \raggedright $\misere@buildpresent#4,@\>$
  \end{array}
}

\def\misere@buildpresent#1=#2,#3{
  {\misere@parseword#1@=\misere@parseword#2@}
  \ifx#3@
    \let\next=\relax
    \let\nextt=\relax
  \else
    ,\ \allowbreak
    \let\next=\misere@buildpresent
    \let\nextt=#3
  \fi
  \next\nextt
}

\def\misere@parseword#1{
  #1
  \misere@parserestofword
}

\def\misere@parserestofword#1{
  \ifx#1@
    \let\next=\relax
  \else\ifcat#1a
    #1
    \let\next=\misere@parserestofword
  \else
    ^{#1}
    \let\next=\misere@parserestofword
  \fi\fi
  \next
}

\newcommand{\centeredplist}[3][c]{
  \parbox[#1]{#2}{\centering $\{\misere@buildplist#3,@\}$}
}

\newcommand{\plist}[3][c]{
  \parbox[#1]{#2}{\raggedright $\{\misere@buildplist#3,@\}$}
}

\def\misere@buildplist#1,#2{
  \misere@parseword#1@
  \ifx#2@
    \let\next=\relax
    \let\nextt=\relax
  \else
    ,\allowbreak
    \let\next=\misere@buildplist
    \let\nextt=#2
  \fi
  \next\nextt
}

\newcounter{misere@cnt}
\newcounter{misere@pcnt}
\newcounter{misere@period}

\newcommand{\cpretend}[1]{
  \misere@buildcpre#1 @ 
}

\def\misere@buildcpre#1 {
  \ifx#1@
    \let\next=\cdots
  \else
    \misere@parseword#1@\ \allowbreak
    \let\next=\misere@buildcpre
  \fi
  \next
}

\newcommand{\pretend}[2]{
  \def\misere@showrownumber{\arabic{misere@cnt}+}
  \def\misere@processpreentry##1@{##1}
  \def\misere@putcdots{& \multicolumn{2}{c}{\cdots}}
  $\begin{array}{r|cccccccccccccccccccccccccccccccccc}
  \misere@prehdr{#1}
  \\ \hline
  \misere@pre{#1}{#2}
  \end{array}$
}


\newcommand{\xpretend}[2]{
  \def\misere@showrownumber{\arabic{misere@cnt}+}
  \let\misere@processpreentry=\misere@parseword
  \def\misere@putcdots{& \multicolumn{2}{c}{\cdots}}
  $\begin{array}{r|cccccccccccccccccccccccccccccccccc}
  \misere@prehdr{#1}
  \\ \hline
  \misere@pre{#1}{#2}
  \end{array}$
}

\newcommand{\cxpretend}[2]{
  \def\misere@showrownumber{}
  \let\misere@processpreentry=\misere@parseword
  \def\misere@putcdots{& \multicolumn{3}{c}{\cdots}}
  $\begin{array}{@{}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{~}c@{}}
  \misere@pre{#1}{#2}
  \end{array}$
}

\newcommand{\misere@prehdr}[1]{
  \setcounter{misere@period}{#1}
  \setcounter{misere@cnt}{1}
  \misere@buildprehdr
}

\def\misere@buildprehdr{
  & \arabic{misere@cnt}
  \stepcounter{misere@cnt}
  \ifnum\arabic{misere@cnt}>\arabic{misere@period}
    \let\next=\relax
  \else
    \let\next=\misere@buildprehdr
  \fi
  \next
}

\newcommand{\misere@pre}[2]{
  \setcounter{misere@period}{#1}
  \setcounter{misere@cnt}{0}
  \setcounter{misere@pcnt}{0}
  \misere@buildpre#2 @ 
}

\def\misere@buildpre#1 {
  \ifx#1@
    \let\next=\misere@putcdots
  \else
    \misere@processpre{#1}
    \let\next=\misere@buildpre
  \fi
  \next
}

\def\misere@processpre#1{%
  \ifnum\arabic{misere@pcnt}=\arabic{misere@period}
    \setcounter{misere@pcnt}{0}
  \fi
  \ifnum\arabic{misere@pcnt}=0
    \ifnum\arabic{misere@cnt}>0
      \\
    \fi
    \misere@showrownumber
  \fi
  & \misere@processpreentry#1@
  \stepcounter{misere@cnt}
  \stepcounter{misere@pcnt}
}

\newcounter{misere@pdnrows}
\newcounter{misere@pdncols}
\newcounter{misere@pdgridheight}
\newcounter{misere@pdgridwidth}
\newcounter{misere@pdrow}
\newcounter{misere@pdcol}
\newcounter{misere@pdx}
\newcounter{misere@pdy}
\newcounter{misere@pdval}

\newcommand{\pdiagram}[3]{
  \setcounter{misere@pdnrows}{#1}
  \setcounter{misere@pdncols}{#2}
  \setcounter{misere@pdgridheight}{6*#1}
  \setcounter{misere@pdgridwidth}{6*#2}
  \setcounter{misere@pdx}{6*#2}
  \setcounter{misere@pdy}{6*#1+10}
  \begin{picture}(\arabic{misere@pdx},\arabic{misere@pdy})
  \multiput(0,0)(0,6){\arabic{misere@pdnrows}}{\line(1,0){\arabic{misere@pdgridwidth}}}
  \multiput(0,0)(6,0){\arabic{misere@pdncols}}{\line(0,1){\arabic{misere@pdgridheight}}}
  \put(0,\arabic{misere@pdgridheight}){\line(1,0){\arabic{misere@pdgridwidth}}}
  \put(\arabic{misere@pdgridwidth},0){\line(0,1){\arabic{misere@pdgridheight}}}
  \setcounter{misere@pdrow}{0}
  \setcounter{misere@pdcol}{0}
  \misere@buildpdcolticks
  \misere@buildpdrowticks
  \setcounter{misere@pdrow}{0}
  \setcounter{misere@pdcol}{0}
  \misere@buildpd #3 @
  \end{picture}
}

\def\misere@buildpdcolticks{
  \ifnum\arabic{misere@pdcol}=\arabic{misere@pdncols}
    \let\next=\relax
  \else
    \setcounter{misere@pdx}{6*\arabic{misere@pdcol}+1}
    \setcounter{misere@pdy}{\arabic{misere@pdgridheight}+2}
    \ifnum\arabic{misere@pdcol}>9 \setcounter{misere@pdval}{\arabic{misere@pdcol}-10}
    \else\setcounter{misere@pdval}{\arabic{misere@pdcol}}\fi
    \put(\arabic{misere@pdx},\arabic{misere@pdy}){\scriptsize \arabic{misere@pdval}}%
    \stepcounter{misere@pdcol}
    \let\next=\misere@buildpdcolticks
  \fi
  \next
}

\def\misere@buildpdrowticks{
  \ifnum\arabic{misere@pdrow}=\arabic{misere@pdnrows}
    \let\next=\relax
  \else
    \setcounter{misere@pdx}{-6}
    \setcounter{misere@pdy}{\arabic{misere@pdgridheight}-5-6*\arabic{misere@pdrow}}
    \ifnum\arabic{misere@pdrow}>9 \setcounter{misere@pdval}{\arabic{misere@pdrow}-10}
    \else\setcounter{misere@pdval}{\arabic{misere@pdrow}}\fi
    \put(\arabic{misere@pdx},\arabic{misere@pdy}){\scriptsize \arabic{misere@pdval}}
    \stepcounter{misere@pdrow}
    \let\next=\misere@buildpdrowticks
  \fi
  \next
}

\def\misere@buildpd #1{
  \ifx#1@
    \let\next=\relax
  \else
    \misere@processpd{#1}
    \let\next=\misere@buildpd
  \fi
  \next
}

\def\misere@processpd#1{
  \ifnum\arabic{misere@pdcol}=\arabic{misere@pdncols}
    \setcounter{misere@pdcol}{0}
    \stepcounter{misere@pdrow}
  \fi
  \ifx#1P
    \setcounter{misere@pdx}{3+6*\arabic{misere@pdcol}}
    \setcounter{misere@pdy}{\arabic{misere@pdgridheight}-3-6*\arabic{misere@pdrow}}
    \put(\arabic{misere@pdx},\arabic{misere@pdy}){\circle*{4}}
  \else
  \ifx#1o
    \setcounter{misere@pdx}{3+6*\arabic{misere@pdcol}}
    \setcounter{misere@pdy}{\arabic{misere@pdgridheight}-3-6*\arabic{misere@pdrow}}
    \put(\arabic{misere@pdx},\arabic{misere@pdy}){\circle{4}}
  \else
  \ifx#1.\relax
  \else
    \setcounter{misere@pdx}{1+6*\arabic{misere@pdcol}}
    \setcounter{misere@pdy}{\arabic{misere@pdgridheight}-4-6*\arabic{misere@pdrow}}
    \put(\arabic{misere@pdx},\arabic{misere@pdy}){\scriptsize #1}
  \fi\fi\fi
  \stepcounter{misere@pdcol}
}

\newcommand{\ijlabel}[2]{%
\begin{minipage}[b]{1cm}%
$\begin{array}{@{}r@{~}l@{}}%
i & \mathrm{#1}\\ j & \mathrm{#2}%
\end{array}$

\vspace{1.5cm}~
\end{minipage}
}

\makeatother

